MonoSparse-CAM: Efficient Tree Model Processing via Monotonicity and Sparsity in CAMs

While the tree-based machine learning (TBML) models exhibit superior performance compared to neural networks on tabular data and hold promise for energy-efficient acceleration using aCAM arrays, their ideal deployment on hardware with explicit exploitation of TBML structure and aCAM circuitry remains a challenging task. In this work, we present MonoSparse-CAM, a new CAM-based optimization technique that exploits TBML sparsity and monotonicity in CAM circuitry to further advance processing performance. Our results indicate that MonoSparse-CAM reduces energy consumption by upto to 28.56x compared to raw processing and by 18.51x compared to state-of-the-art techniques, while improving the efficiency of computation by at least 1.68x.

==> referenceslist.tex <==

\begin{thebibliography}{00}

\bibitem{AIintro1} LeCun, Y., Bengio, Y., Hinton, G. Deep learning. Nature 521, 436–444 (2015). https://doi.org/10.1038/nature14539 % general paper on DL

\bibitem{AIintro2} Pedro AR, Dias MB, Laranjo L, Cunha AS, Cordeiro JV. Artificial intelligence in medicine: A comprehensive survey of medical doctor's perspectives in Portugal. PLoS One. 2023 Sep 7;18(9):e0290613. doi: 10.1371/journal.pone.0290613. PMID: 37676884; PMCID: PMC10484446. % AI in healthcare

\bibitem{AIintro3} Bi, Ying , Xue, Bing , Mesejo, Pablo , Cagnoni, Stefano , Zhang, Mengjie. (2022). A Survey on Evolutionary Computation for Computer Vision and Image Analysis: Past, Present, and Future Trends. IEEE Transactions on Evolutionary Computation. PP. 1-1. 10.1109/TEVC.2022.3220747.  % AI in CV




% tabular is the most common data type
\bibitem{tabulariscommon1} Liu, D. et al. (2023, April). DIWIFT: Discovering Instance-wise Influential Features for Tabular Data. In Proceedings of the ACM Web Conference 2023 (pp. 1673-1682).
\bibitem{tabulariscommon2} Luo, Y., Zhou, H., Tu, W. W., Chen, Y., Dai, W., and Yang, Q. (2020, July). Network on network for tabular data classification in real-world applications. In Proceedings of the 43rd International ACM SIGIR Conference on Research and Development in Information Retrieval (pp. 2317-2326).



\bibitem{GreenAI} R. Schwartz, J. Dodge, N. A. Smith, and O. Etzioni, “Green AI,” Communications of the ACM, December 2020, Vol. 63 No. 12, Pages 54-63
10.1145/3381831

% TBML > DL models on tabular data
\bibitem{DL_tabular} Borisov, Vadim et al. “Deep Neural Networks and Tabular Data: A Survey.” IEEE transactions on neural networks and learning systems PP (2021): n. pag. % DNN on tabular
\bibitem{PyTorchTabular} Joseph, Manu. "Pytorch tabular: A framework for deep learning with tabular data." arXiv preprint arXiv:2104.13638 (2021).
\bibitem{TabularIntoImages} Zhu, Y., Brettin, T., Xia, F. et al. Converting tabular data into images for deep learning with convolutional neural networks. Sci Rep 11, 11325 (2021). https://doi.org/10.1038/s41598-021-90923-y
\bibitem{LocalGLMnet} Richman, Ronald, and Mario V. Wüthrich. "LocalGLMnet: interpretable deep learning for tabular data." Scandinavian Actuarial Journal 2023.1 (2023): 71-95.



\bibitem{TBML>DL1} L. Grinsztajn, E. Oyallon, and G. Varoquaux, "Why do tree-based models still outperform deep learning on typical tabular data?," Thirty-sixth Conference on Neural Information Processing Systems Datasets and Benchmarks Track, 2022.
\bibitem{TBML>DL2} R. Shwartz-Ziv and A. Armon, “Tabular Data: Deep Learning is Not All You Need,” 8th ICML Workshop on Automated Machine Learning (AutoML), Jul. 14, 2021.
\bibitem{TBML>DL3} Yury Gorishniy, I. Rubachev, V. Khrulkov, and A. Babenko, “Revisiting Deep Learning Models for Tabular Data,” Advances in Neural Information Processing Systems, Volume 34, 2-21, 18932--18943. % GBDT is still beating NN

\bibitem{TBML>DL4} Lindskog, William, and Christian Prehofer. "A Federated Learning Benchmark on Tabular Data: Comparing Tree-Based Models and Neural Networks." 2023 Eighth International Conference on Fog and Mobile Edge Computing (FMEC). IEEE, 2023. % even for federated learning TBM > DNN
\bibitem{TBML>DL5} Ullah, Zahid, et al. "Comparison of tree-based model with deep learning model in predicting effluent pH and concentration by capacitive deionization." Desalination 558 (2023): 116614. % cost effectiveness. 100 times less than the DL model) with almost the same prediction accuracy


% pedretti papers. for feature reordering argument
\bibitem{b2} Pedretti, Giacomo, et al. "Tree-based machine learning performed in-memory with memristive analog CAM." Nature communications 12.1 (2021): 5806. %feature reordering paper

\bibitem{energypercell} Li, C., Graves, C.E., Sheng, X. et al. Analog content-addressable memories with memristors. Nat Commun 11, 1638 (2020). https://doi.org/10.1038/s41467-020-15254-4 % energy consumption calculations




% papers on CAM circuits
\bibitem{b3} Graves, Catherine E., et al. "In‐memory computing with memristor content addressable memories for pattern matching." Advanced Materials 32.37 (2020): 2003437. %4t2m paper
\bibitem{b4} Bahloul, Mohamed A., et al. "Design and analysis of 2T-2M ternary content addressable memories." 2017 IEEE 60th International Midwest Symposium on Circuits and Systems (MWSCAS). IEEE, 2017.  %2t2m paper
\bibitem{b5}  Bazzi, Jinane, et al. "Efficient analog cam design." arXiv preprint arXiv:2203.02500 (2022). %various circuits


% matching techniques
\bibitem{b6} Hu, Xiaobo Sharon, et al. "In-memory computing with associative memories: A cross-layer perspective." 2021 IEEE International Electron Devices Meeting (IEDM). IEEE, 2021. %different matching techniques

\bibitem{b7} 

\end{thebibliography}

==> sections/0author.tex <==
\author{\IEEEauthorblockN{Tergel Molom-Ochir}
\IEEEauthorblockA{Duke University \\
Durham, North Carolina, USA \\
tergel.molom-ochir@duke.edu}
\and
\IEEEauthorblockN{Brady Taylor}
\IEEEauthorblockA{Duke University \\
Durham, North Carolina, USA \\
brady.g.taylor@duke.edu}
\and
\IEEEauthorblockN{Hai (Helen) Li}
\IEEEauthorblockA{Duke University \\
Durham, North Carolina, USA \\
hai.li@duke.edu}
\and
\IEEEauthorblockN{Yiran Chen}
\IEEEauthorblockA{Duke University \\
Durham, North Carolina, USA \\
yiran.chen@duke.edu}

}

==> sections/methodology3.tex <==


 With a constant size of 24x48, total energy and delay for $\lambda$ values from 0.1 to 0.5 are the same as at $\lambda$=0.5. 
 Therefore, Fig. 4a-c focus on $\lambda$ values from 0.5 to 0.9.



%With constant height and width sizes of 24x48, for $\lambda$ values from 0.1 to 0.5, the total energy and delay are the same as at $\lambda$ = 0.5. Therefore, Fig. \ref{subfig:energy_consumption_comparison}, \ref{subfig:delay_comparison}, and \ref{subfig:computational_efficiency_comparison} focus on $\lambda$ values from 0.5 to 0.9.


%Due to the availability of computational resources, CAM width and height sizes up to 64 and up to three trials were simulated.
